A note on two notions of compliance

We establish a relation between two models of contracts: binary session types, and a model based on event structures and game-theoretic notions. In particular, we show that compliance in session types corresponds to the existence of certain winning strategies in game-based contracts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{86}
\providecommand{\publicationstatus}{I. Lanese, A. Lluch Lafuente, A. Sokolova, H. T. Vieira (Eds.):\\
7th Interaction and Concurrency Experience (ICE 2014)\\
EPTCS 166, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.166.9}{10.4204/EPTCS.166.9}}
\pdfoutput=1

